A Geometric Approach to Online Streaming Feature Selection

Online Streaming Feature Selection (OSFS) is a sequential learning problem where individual features across all samples are made available to algorithms in a streaming fashion. In this work, firstly, we assert that OSFS's main assumption of having data from all the samples available at runtime is unrealistic and introduce a new setting where features and samples are streamed concurrently called OSFS with Streaming Samples (OSFS-SS). Secondly, the primary OSFS method, SAOLA utilizes an unbounded mutual information measure and requires multiple comparison steps between the stored and incoming feature sets to evaluate a feature's importance. We introduce Geometric Online Adaption, an algorithm that requires relatively less feature comparison steps and uses a bounded conditional geometric dependency measure. Our algorithm outperforms several OSFS baselines including SAOLA on a variety of datasets. We also extend SAOLA to work in the OSFS-SS setting and show that GOA continues to achieve the best results. Thirdly, the current paradigm of the OSFS algorithm comparison is flawed. Algorithms are measured by comparing the number of features used and the accuracy obtained by the learner, two properties that are fundamentally at odds with one another. Without fixing a limit on either of these properties, the qualities of features obtained by different algorithms are incomparable. We try to rectify this inconsistency by fixing the maximum number of features available to the learner and comparing algorithms in terms of their accuracy. Additionally, we characterize the behaviour of SAOLA and GOA on feature sets derived from popular deep convolutional featurizers.

==> Proofs_Lemmas.tex <==
\section{Proof of Lemmas}

\subsection{Proof of Lemma 3.2:}
Given $p\in(0,1)$ and $q=1-p$, we can easily check that for positive $t>q$, $s>q$, such that $t,s\neq 1$:
$$(t+s)\left[(ts)+q(1-t-s)\right]-p (ts)\geq 0.$$
This implies
\begin{equation}\label{eq.1}
p\Big(\diy\frac{t-q}{p}\Big)\Big(\frac{s-q}{p}\Big)+q\geq \diy\frac{t\;s}{t+s}.\end{equation}
In (\ref{eq.1}), substitute 
$$\frac{s-q}{p}=\frac{f(F_i,c;x)}{f(F_i,c) f(x)},\;\; \frac{t-q}{p}=\frac{f(x)}{f(x|c)},$$
therefore the LHS in (\ref{eq.1}) becomes 
$$p\left(\frac{f(F_i,c;x)}{f(F_i,c) f(x)}\right)\left(\frac{f(x)}{f(x|c)}\right)+q=p\left(\frac{f(F_i,x|c)}{f(F_i|c)f(x|c)}\right)+q.$$
Set $p=q=1/2$, hence by conditional mutual information definition in \cite{ICASSPsalimeh2019}, we have 
\begin{equation}\label{eq.2}
I(F_i;X|C)\geq 1-\bbE_f\left[\frac{1}{s}\right]-\bbE_f\left[\frac{1}{t}\right],
\end{equation}
where $1-\diy\bbE_f\left[s^{-1}\right]=I(F_i,C;X)$ and
\begin{equation}\label{eq.3}
\bbE_f\left[t^{-1}\right]=2\bbE_f\left[\left(\frac{f(X)}{f(X|C)}+1\right)^{-1}\right].
\end{equation}
Combine (\ref{eq.2}) and (\ref{eq.3}). This implies our claim inequality (3) in Lemma 3.2. 


\subsection{\bf Proof of Lemma 3.3:} 


From assumption (4) in Lemma 3.3, we can get that $\exists \bar{\delta}\geq 0$ such that for all $\epsilon\geq 0$
\begin{equation}
\left(\frac{1}{f(F_i|x)f(c|x)}+\epsilon\right)^{-1}-\left(\frac{1}{f(F_i)f(c)}+\epsilon\right)^{-1}\geq \bar{\delta}.
\end{equation}
Now set $\epsilon=\left(f(F_i,c|x)\right)^{-1}$, then $\exists \tilde{\delta}\geq 0$ such that
\begin{equation}\label{eq.6}
\bbE_f\left[\left(\frac{f(F_i,C|X)}{f(F_i|X)f(C|X)}+1\right)^{-1}-\left(\frac{f(F_i,C|X)}{f(F_i)f(C)}+1\right)^{-1}\right]\geq \tilde{\delta}.
\end{equation}
On the other hand we discard $F_i$ if $f(c|F_i)=f(c)$ and $f(c|x,F_i)=f(c|x)$ for $x\in S^*_{t_{i-1}}$. This implies $f(F_i,c)=f(F_i)f(c)$, therefore the LHS in (\ref{eq.6}) becomes
\begin{equation}\label{eq.7}
\bbE_f\left[\left(\frac{f(F_i,C|X)}{f(F_i|X)f(C|X)}+1\right)^{-1}-\left(\frac{f(F_i,C,X)}{f(F_i,C)f(X)}+1\right)^{-1}\right]
\end{equation}
The term (\ref{eq.7}) equals $I(F_i,C;X)-I(F_i;C|X)$, consequently going back to (\ref{eq.6}), $\exists {\tilde{\delta}}\geq 0$ such that
\begin{equation}
I(F_i,C;X)-I(F_i;C|X)\geq \tilde{\delta}.
\end{equation}
This completes the proof of Lemma 3.3. 


==> writing/introduction.tex <==
Let us motivate the field of Feature Selection (FS) with a simple example. Consider a doctor diagnosing a patient with disease; given the patient's health history and test results, the doctor will focus on relevant pieces of information to make her final diagnosis. This usage of a subset of the information available in the decision making process inspires the field of FS~\cite{tibshirani1996regression,kohavi1997wrappers,dash2003consistency,yu2003feature}. By limiting the number of features required to perform a task, FS allows for the training of faster models that utilize lower computational and storage requirements while ideally achieving similar performance to working with all the features. 

Now consider an extension to the previous example to motivate Online Streaming Feature Selection (OSFS). Imagine the patient was admitted to the ER and it is imperative that a reliable diagnosis is made quickly. The doctor is likely to order several tests and use the most informative results to refine her decision. This usage of information as it is made available inspires Online Streaming Feature Selection (OSFS)~\cite{Zhouetal2005,wu2010online}. In OSFS, individual features across all samples are made available to algorithms in streaming fashion. Algorithms are allowed a single pass at the new features and are tasked with  maintaining a list of decision-relevant features by disregarding uninformative old ones (i.e. measuring feature redundancy) and incorporating informative new ones(i.e. measuring feature relevancy). 

\citet{Zhouetal2005} introduced the alpha-investing algorithm as one of the earliest solutions to the OSFS problem. 
Here new features are added to the minimal subset via dynamic thresholding of a p-statistic between current features and incoming features. 
\citet{wu2010online} and it's subsequent work  \citet{Wuetal.2013} introduce concepts of feature relevance and redundancy to prune and maintain small subsets of features for this task. 
Their algorithms perform local comparisons between incoming features and the current feature and global comparisons between the minimal subset collected thus far with the incoming feature. 
SAOLA(Scalable and Accurate Online feature selection) ~\cite{Yuetal2014} approaches the problem by measuring intra-feature redundancy and dependency using mutual information (MI)\cite{Cover1991ElementsOI}. 
However, the histogram estimator used in SAOLA imposes improper bounds for thresholding and they have multiple comparison steps across their algorithm which makes it inefficient.

Our first contribution is the creation of the Geometric Online Adaption (GOA) algorithm. 
The algorithm uses \citet{ICASSPsalimeh2019}'s new class-conditional graph-based geometric dependency measure (CGD) to calculate intra-feature relevancy and redundancy. 
Under GOA's assumptions, we show that there exists a feature in the current optimal feature subset such that if the new incoming feature is irrelevant to the class label given that feature, then both the given and incoming feature are dependent. We validate our method against the algorithms described above across multiple datasets.

For our second contribution, we assert that OSFS's assumption of having data from all the samples available at runtime is unrealistic. 
In our doctor example, consider that more patients were admitted to the ER exhibiting similar symptoms to the previous patient. It is likely that the doctor would use the prior information to jumpstart diagnoses while evaluating patients' new test results as well. Based on this assertion, we extend OSFS to a new setting called Online Streaming Feature Selection with Streaming Samples (OSFS-SS), where both samples and features are streamed concurrently. We experiment with a variety of different sample set sizes at different time steps, the details of which can be found in our methodology section (Fig.~\ref{fig.Scenarios}). 

%Based on this intuition, we assert that expecting all the samples to be available at start time is an unrealistic assumption. We experiment with three different variants of the new OSFS-SS setting: (a) at every new time-step, the algorithms are presented with new sample sets where the size of the sets from time-step to time-step is held constant (b) at every new time-step, algorithms are presented with sample sets of different sizes and (c) while at different time-steps, the size of the sample sets remain the same, individual features may be repeated from one set to the next one (e.g. standard practice in most hospitals is to measure a patients vital signs on arrival).

Our third contribution is to augment OSFS algorithms to the OSFS-SS setting. We extend SAOLA to work with streaming samples using it as a baseline. We also show how GOA is naturally suited to the new setting requiring minimal changes. GOA achieves state-of-the-art results on the OSFS-SS setting outperforming SAOLA on most datasets.
The new streaming setting also us to apply algorithms to features derived from publicly available convolutional neural network (CNN) featurizers. We are interested in testing the presence of redundancy in these deep featurizers and evaluating how they are different from the human-annotated feature sets that normally dominate this line of work. 
% We characterize the behaviour of SAOLA and GOA on these feature sets which indicate a divergent property between their response to non-CNN and CNN-based features.

%Our fourth contribution is to extend the OSFS-SS setting to use deep features sets derived from a variety of popular and publicly available convolutional neural networks. Note that the output of CNN-based feature vectors are high dimensional - as a result, it is the streaming samples setting that allows us to operate on these high dimensional vectors. The original OSFS setting requires the computation of the entire data matrix in memory making it difficult to perform these deep experiments. We believe these experiments are important as with the advent and popularity of deep learning methods in machine learning, we wish to gain an understanding for how much redundancy may be present within the feature outputs of convolutional neural networks. 

==> writing/osfs_algorithms.tex <==



 
 \subsection{Setup: OSFS with Streaming Samples}
 \label{subsec:osfsss}
  \input{writing/osfss-ss}
\newpage
\subsection{Geometric Online Adaptation}
 \label{subsec:goa}
 \input{writing/goa}
 
\subsection{Fair Comparison against Baseline} 
 To ensure fair performance comparisons across baselines and datasets we choose to constrain our algorithm to always use $\delta$ values that correspond to smaller feature subsets than the baseline against which GOA is being compared, i.e., the GOA results are to be comparatively assessed w.r.t. a baseline. 
 More specifically, we perform a grid search of $\delta$ and select the case which corresponds to the highest accuracy when the selected number of features is lower than or equal to the number of features selected by the baseline being compared against.
 In case GOA does not select a lesser number of features than the baseline, we select the hyper-parameter which corresponds to the closest number of features greater than the baseline, regardless of the performance.
